PalimpChat: Declarative and Interactive AI analytics

Thanks to the advances in generative architectures and large language models, data scientists can now code pipelines of machine-learning operations to process large collections of unstructured data. Recent progress has seen the rise of declarative AI frameworks (e.g., Palimpzest, Lotus, and DocETL) to build optimized and increasingly complex pipelines, but these systems often remain accessible only to expert programmers. In this demonstration, we present PalimpChat, a chat-based interface to Palimpzest that bridges this gap by letting users create and run sophisticated AI pipelines through natural language alone. By integrating Archytas, a ReAct-based reasoning agent, and Palimpzest's suite of relational and LLM-based operators, PalimpChat provides a practical illustration of how a chat interface can make declarative AI frameworks truly accessible to non-experts. Our demo system is publicly available online. At SIGMOD'25, participants can explore three real-world scenarios--scientific discovery, legal discovery, and real estate search--or apply PalimpChat to their own datasets. In this paper, we focus on how PalimpChat, supported by the Palimpzest optimizer, simplifies complex AI workflows such as extracting and analyzing biomedical data.

==> code/agent_tools.tex <==
\begin{table}[t]
\scriptsize
\centering
\label{tab:agent_tools_short}
\begin{tabular}{p{2.0cm}p{5.1cm}}
\toprule
\textbf{Tool} & \textbf{Description} \\
\midrule

\texttt{register\_dataset} 
& \textbf{Inputs:} (\texttt{path} (str), \texttt{name} (str)) 
\newline \textbf{Function:} Register a dataset for subsequent use. \\[5pt]

\texttt{unregister\_dataset}
& \textbf{Inputs:} (\texttt{dataset\_name} (str))
\newline \textbf{Function:} Remove a dataset from the system. \\[5pt]

\texttt{list\_datasets}
& \textbf{Inputs:} None  
\newline \textbf{Function:} Show all tracked datasets. \\[5pt]

\texttt{retrieve\_dataset}
& \textbf{Inputs:} (\texttt{dataset\_path} (str)) 
\newline \textbf{Function:} List records in a dataset. \\[5pt]

\texttt{generate\_extraction\_}\\ \texttt{schema}
& \textbf{Inputs:} (\texttt{schema\_name}, \texttt{schema\_description}, \texttt{field\_names}, \texttt{field\_descriptions}, \texttt{field\_required})
\newline \textbf{Function:} Define a new schema for extracting fields. \\[5pt]

\texttt{filter\_data}
& \textbf{Inputs:} (\texttt{input\_dataset} (str), \texttt{filter\_expression} (str))
\newline \textbf{Function:} Filter a dataset using a natural-language condition. \\[5pt]

\texttt{convert\_dataset}
& \textbf{Inputs:} (\texttt{input\_dataset}, \texttt{schema}, \texttt{cardinality})
\newline \textbf{Function:} Transform a dataset into a new schema. \\[5pt]

\texttt{override\_dataset}
& \textbf{Inputs:} (\texttt{input\_dataset} (str))
\newline \textbf{Function:} Reset the current “active” dataset. \\[5pt]

\texttt{set\_input\_dataset}
& \textbf{Inputs:} (\texttt{dataset} (str), \texttt{input\_schema} (str))
\newline \textbf{Function:} Establish a default dataset and schema. \\[5pt]

\texttt{pick\_schema}
& \textbf{Inputs:} (\texttt{schema\_name} (str))
\newline \textbf{Function:} Retrieve (or create) a named schema. \\[5pt]

\texttt{list\_schemas}
& \textbf{Inputs:} None
\newline \textbf{Function:} Show all known schemas. \\[5pt]

\texttt{execute\_workload}
& \textbf{Inputs:} (\texttt{output\_dataset}, \texttt{policy\_method}, \texttt{allow\_code\_synth}, \texttt{allow\_token\_reduction})
\newline \textbf{Function:} Execute a pipeline under a chosen policy. \\
\bottomrule
\end{tabular}
\caption{Core \chat\ Tools.}
\end{table}

==> code/all_tools.tex <==

% \paragraph{1.\ \texttt{register\_dataset}}
% \begin{itemize}
% \item \textbf{Inputs:} 
%   \begin{itemize}
%   \item \texttt{path} (string): File or directory path to be registered.
%   \item \texttt{name} (string): Name to assign to the dataset.
%   \end{itemize}
% \item \textbf{Output:} 
%   \begin{itemize}
%   \item \texttt{str}: A message indicating the registration status.
%   \end{itemize}
% \item \textbf{Functionality:} 
%   Registers a dataset in the \sys\ system so it can be used in later steps, such as filtering or schema-based transformations.
% \end{itemize}

% \paragraph{2.\ \texttt{unregister\_dataset}}
% \begin{itemize}
% \item \textbf{Inputs:}
%   \begin{itemize}
%   \item \texttt{dataset\_name} (string): Name of the dataset to unregister.
%   \end{itemize}
% \item \textbf{Output:} 
%   \begin{itemize}
%   \item \texttt{str}: A message about the unregistration result.
%   \end{itemize}
% \item \textbf{Functionality:} 
%   Removes a dataset from \sys\ so it is no longer accessible.
% \end{itemize}

% \paragraph{3.\ \texttt{list\_datasets}}
% \begin{itemize}
% \item \textbf{Inputs:} None.
% \item \textbf{Output:} 
%   \begin{itemize}
%   \item \texttt{str}: A formatted list of all registered datasets.
%   \end{itemize}
% \item \textbf{Functionality:} 
%   Provides an overview of all currently tracked datasets in the system.
% \end{itemize}

% \paragraph{4.\ \texttt{retrieve\_dataset}}
% \begin{itemize}
% \item \textbf{Inputs:}
%   \begin{itemize}
%   \item \texttt{dataset\_path} (string): Location of the dataset in \sys.
%   \end{itemize}
% \item \textbf{Output:}
%   \begin{itemize}
%   \item \texttt{list[str]}: A list of item identifiers (filenames, keys, etc.) contained in the dataset.
%   \end{itemize}
% \item \textbf{Functionality:}
%   Shows which records (e.g., individual documents) are available in a particular dataset.
% \end{itemize}

% \paragraph{5.\ \texttt{generate\_extraction\_schema}}
% \begin{itemize}
% \item \textbf{Inputs:}
%   \begin{itemize}
%   \item \texttt{schema\_name} (string): Name for the new schema.
%   \item \texttt{schema\_description} (string): Description for the intended schema.
%   \item \texttt{field\_names} (list): List of attribute names.
%   \item \texttt{field\_descriptions} (list): Descriptions corresponding to each field name.
%   \item \texttt{field\_required} (list): Boolean flags indicating required attributes.
%   \end{itemize}
% \item \textbf{Output:} 
%   \begin{itemize}
%   \item \texttt{str}: The name of the newly created schema.
%   \end{itemize}
% \item \textbf{Functionality:}
%   Defines a new schema that can be subsequently used for extracting named attributes from unstructured data.
% \end{itemize}


% \paragraph{6.\ \texttt{filter\_data}}
% \begin{itemize}
% \item \textbf{Inputs:}
%   \begin{itemize}
%   \item \texttt{input\_dataset} (string): The dataset to filter.
%   \item \texttt{filter\_expression} (string): A natural-language condition describing which records to keep.
%   \end{itemize}
% \item \textbf{Output:}
%   \begin{itemize}
%   \item \texttt{str}: A new dataset containing only the records that match the given condition.
%   \end{itemize}
% \item \textbf{Functionality:}
%   Harnesses LLMs or other methods to parse the user’s filter expression and apply the appropriate subset operation on the dataset.
% \end{itemize}

% \paragraph{7.\ \texttt{convert\_dataset}}
% \begin{itemize}
% \item \textbf{Inputs:}
%   \begin{itemize}
%   \item \texttt{input\_dataset} (string): The source dataset.
%   \item \texttt{schema} (string): The target schema name for conversion.
%   \item \texttt{cardinality} (string): Either \texttt{``one\_to\_one''} or \texttt{``one\_to\_many''}, indicating how many schema objects can be extracted from a single record.
%   \end{itemize}
% \item \textbf{Output:}
%   \begin{itemize}
%   \item \texttt{str}: The newly created dataset under the specified schema.
%   \end{itemize}
% \item \textbf{Functionality:}
%   Transforms the data into a desired form (e.g., extracting specific attributes from documents) by applying the specified schema.  
% \end{itemize}

% \paragraph{8.\ \texttt{override\_dataset}}
% \begin{itemize}
% \item \textbf{Inputs:}
%   \begin{itemize}
%   \item \texttt{input\_dataset} (string): The dataset to become the new working dataset.
%   \end{itemize}
% \item \textbf{Output:}
%   \begin{itemize}
%   \item \texttt{str}: Confirmation of the newly set working dataset.
%   \end{itemize}
% \item \textbf{Functionality:}
%   Resets the current environment’s notion of the ``active'' dataset to the specified dataset, which is useful after an extraction or other transformations.
% \end{itemize}

% \paragraph{9.\ \texttt{set\_input\_dataset}}
% \begin{itemize}
% \item \textbf{Inputs:}
%   \begin{itemize}
%   \item \texttt{dataset} (string): Name of the dataset to set as input.
%   \item \texttt{input\_schema} (string): Name of the schema to apply when loading; if unknown, the tool attempts to find or create a matching schema.
%   \end{itemize}
% \item \textbf{Output:}
%   \begin{itemize}
%   \item \texttt{str}: The dataset now set as the input for subsequent operations.
%   \end{itemize}
% \item \textbf{Functionality:}
%   Establishes or updates the default dataset and schema for a \sys\ pipeline before initiating further actions.
% \end{itemize}

% \paragraph{10.\ \texttt{pick\_schema}}
% \begin{itemize}
% \item \textbf{Inputs:}
%   \begin{itemize}
%   \item \texttt{schema\_name} (string): The name of the desired schema.
%   \end{itemize}
% \item \textbf{Output:}
%   \begin{itemize}
%   \item \texttt{str}: The identified schema object or \texttt{None} if not found.
%   \end{itemize}
% \item \textbf{Functionality:}
%   Retrieves an existing schema by name, or indicates the need to create a new one if none is found.
% \end{itemize}

% \paragraph{11.\ \texttt{list\_schemas}}
% \begin{itemize}
% \item \textbf{Inputs:} None.
% \item \textbf{Output:}
%   \begin{itemize}
%   \item \texttt{str}: A formatted overview of all known schemas in the system.
%   \end{itemize}
% \item \textbf{Functionality:}
%   Displays which schemas are available for tasks such as conversions and extractions.
% \end{itemize}

% \paragraph{12.\ \texttt{execute\_workload}}
% \begin{itemize}
% \item \textbf{Inputs:}
%   \begin{itemize}
%   \item \texttt{output\_dataset} (string): The dataset on which the final extraction or transformation should run.
%   \item \texttt{policy\_method} (string): Specifies whether to prioritize cost (\texttt{min\_cost}) or quality (\texttt{max\_quality}).
%   \item \texttt{allow\_code\_synth} (string): Enables or disables code synthesis (\texttt{``True''} or \texttt{``False''}).
%   \item \texttt{allow\_token\_reduction} (string): Enables or disables token reduction (\texttt{``True''} or \texttt{``False''}).
%   \end{itemize}
% \item \textbf{Output:}
%   \begin{itemize}
%   \item \texttt{str}: A result summary, typically containing a reference to a Pandas DataFrame with extracted data.
%   \end{itemize}
% \item \textbf{Functionality:}
%   Executes an entire workload on the current pipeline, optionally performing transformations or filtering as needed. The system decides how to run each operator (e.g., LLM-based or conventional) for optimal performance and correctness, based on the user’s preferences.
% \end{itemize}

==> sections/01-intro.tex <==
% \vspace{-10pt}
\section{Introduction} \label{sec:introduction}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/PZ_DEMO.png}
    \caption{An overview of data processing using \sys}
    \label{fig:architecture-overview}
\end{figure}

The advent of generative AI has fundamentally changed how we engage with data and computing systems. Large Language Models (LLMs) now enable a wide range of applications—such as question answering, multimodal and unstructured data extraction, and agent-driven workflows like reasoning and code synthesis~\cite{yao2022react,hong2023metagpt}. However, these systems increasingly rely on intricate architecture: they combine traditional data processing components (e.g., vector databases~\cite{lewis2020retrieval} and relational operators~\cite{palimpzestCIDR}) with novel programming concepts like prompt engineering~\cite{dspy} or multi-step chain-of-thought reasoning.

Such complexity entails several drawbacks. First, the runtime, monetary cost, and resource consumption of AI pipelines can grow exorbitantly. Second, from a software engineering perspective, designing, deploying, and testing these systems is becoming ever more challenging. Developers must juggle a variety of software frameworks and rapidly changing runtime environments, making the promise of “natural language interfaces” increasingly hard to fulfill for complex data processing tasks.

The core challenge to build a declarative data management system for compound AI pipelines is to design an optimizer that can take in logical pipelines as defined by the users, and produce physical implementations of them that meet specific goals in terms of cost, runtime, and output quality.  Furthermore, a technical challenge involves the designing of a user interface to bridge the freedom of expressing general-purpose AI pipelines, as well as imposing a certain structure on the compiled programs in order to perform automated optimization.

To bridge this gap and address these challenges, we present \sys.
Our system is based on a declarative programming framework, that expert users can leverage to build optimized data processing pipelines for large collections of unstructured documents.
On top of this framework, we designed a chat-based assistant \chat\ that allows non-expert users to build their pipelines using natural language.

In this demo, we focus on both interfaces: the native programming environment (for expert developers) and a natural language interface (for less technical users). Our running example tackles a real-world scientific discovery scenario: a medical researcher analyzing literature on cancer-related papers to identify genomic and proteomic datasets that validate specific hypotheses. SIGMOD attendees can also explore two other use cases or upload their own data to design and execute custom pipelines.

\sys\ is an early, but promising, prototype, and we welcome suggestions for further optimizations and features. We encourage readers to consult our extended technical description in~\cite{palimpzestCIDR}, experiment with our open-source \sys{} code at \systemurl, and interact with \chat{} demo at \demourl and code at \chatcode.

The remainder of this paper is structured as follows:  
Section~\ref{sec:architecture} describes the core architecture of \sys\ and the reasoning framework driving \chat.  
Section~\ref{sec:demoscenario} demonstrates a concrete usage scenario through the chat-based interface.

